Soft Robust MDPs and Risk-Sensitive MDPs: Equivalence, Policy Gradient, and Sample Complexity

Robust Markov Decision Processes (MDPs) and risk-sensitive MDPs are both powerful tools for making decisions in the presence of uncertainties. Previous efforts have aimed to establish their connections, revealing equivalences in specific formulations. This paper introduces a new formulation for risk-sensitive MDPs, which assesses risk in a slightly different manner compared to the classical Markov risk measure (Ruszczy\'nski 2010), and establishes its equivalence with a class of soft robust MDP (RMDP) problems, including the standard RMDP as a special case. Leveraging this equivalence, we further derive the policy gradient theorem for both problems, proving gradient domination and global convergence of the exact policy gradient method under the tabular setting with direct parameterization. This forms a sharp contrast to the Markov risk measure, known to be potentially non-gradient-dominant (Huang et al. 2021). We also propose a sample-based offline learning algorithm, namely the robust fitted-Z iteration (RFZI), for a specific soft RMDP problem with a KL-divergence regularization term (or equivalently the risk-sensitive MDP with an entropy risk measure). We showcase its streamlined design and less stringent assumptions due to the equivalence and analyze its sample complexity

==> Response/Further_response_to_reviewer_2__round_1_.tex <==
\section{Further Response to Reviewer RSEz}

\paragraph{The first comment:} 
We would like to sincerely thank the reviewer for the timely response and for giving further suggestions! We now address the reviewer's comments as follows.

We would like to apologize for our misinterpretation of the reviewer's comments in the first round, especially on the term mixture quasi-concave, and for misstating that ``... convex risk measures (referred to as 'quasi-concave/mixture quasi-concave' by the reviewer)''. From the reviewer's new comment and after a more careful checking of the reference Delage et al. [2019], we realize that most of the confusion and miscommunications are due to the different definitions of (convex) risk measures. Before we elaborate on the details, we would like to note that the results in this paper do not conflict with Delage et al. [2019] and Remark 2 (as well as Theorem 2) holds for the convex risk measure defined in the paper. 

First of all, we would like to note that the definition of convex risk measure in Delage et al. is different from the definition of our paper as well as the classical definitions of convex risk measure in literature [29,30,72]. Here we quote the paragraph at the beginning of page 11 in Delage et al. [2019]: 'We alert the reader that we do not implicitly assume convex risk measures to be monetary as is frequently done in the literature. The explicit distinction between convex and convex monetary risk measures will facilitate a more concise description of the main results in this paper.' From the quote, Delage et al. define the risk measure without the monetary assumption, which is the same as the monotonicity property in the definition of convex risk measures in our paper, whereas monotonicity is a necessary property in our definition as well as in the definition of the Markov risk measure [70]. Specifically, the semi-moment risk measures as mentioned by the reviewer 'typically fails to be monotonic (Shapiroetal.2009, Example 6.19)' (quoted from the end of page 17 in Delage et al.). Thus, our statement that the risk-sensitive MDP obtains optimal deterministic policy is not in conflict with the fact that the optimal policy for optimizing semi-moment risk measures might be stochastic, as semi-moment risk measures are not within the discussion of our paper. We have added the above discussion to the footnote after Remark 2. 


Secondly, in Delage et al., they stated that even for convex risk measures without monotonicity, the optimal policy is deterministic as long as the feasible region is convex. (Quote from the introduction: 'deterministic decisions are optimal if both the risk measure and the feasible region are convex, or alternatively if the risk measure is mixture-quasiconcave.') This further corroborates that our results are not in conflict with Delage et al. 

Lastly, we would also like to discuss the relation and difference between the mixture quasiconcavity and convexity. Based on our own understanding of the mixture quasiconcavity (Definition 6 in Delage et al.), a risk measure is mixture quasiconcave if $\rho(\theta X + (1-\theta)Y) \ge \min\{\rho(X), \rho(Y)\}$, which is a different, neither stronger nor weaker, definition compared with convexity.
Thus, neither of the two notions includes the other. A risk measure can be convex but not quasiconcave, and vice versa. For this reason,  our results on convex risk measure with monotonicity do not necessarily apply to mixture-quasiconcave risk measure.

To summarize, we concur with the reviewer that our work has its limitations and could not include convex risk measures without the monotonicity assumption. We also note that our result only holds for convex risk measures with monotonicity instead of mixture quasiconcave risk measures. Accordingly, we have added a footnote in Remark 2 to clearly state that our results hold for convex risk measures with monotonicity; the equivalence might fail if we consider other risk metrics such as semi-moment, where the monotonicity property does not hold. We hope that the above clarifications address the reviewer's concerns. We are happy to further address this if there remains unclearness and misscommunication. 


\paragraph{The second comment:} 
Thank you again for reading our response and giving constructive feedback! 

For point 3), we first thank the reviewer for finding the formulation to be interesting and have attractive properties from the point of view of optimization. We also agree with the reviewer that our work indeed has its limitations, for example, the equivalence of the optimal solution of the risk-sensitive MDP and the Markov risk measure will no longer hold under certain model variations. We have added this limitation into Appendix C in the further revision, here we quote 'However, we would also like to emphasize that when adding policy regularization, the optimal policy might no longer be a deterministic policy. In this setting, the optimal policy and optimal value of the Markov risk measure and the risk-sensitive MDP may not be the same.'

For point 2), we apologize that Remark 2 leaves an inaccurate impression. Due to space limits, we apologize that we could not include a detailed comparison in the main text, thus we defer a more detailed and accurate discussion into Appendix C (highlighted in blue) and further emphasize there that the definition of our risk-sensitive risk measure is different from the Markov risk measure (i.e. denoted as $RPR = \rho(r_1+ \gamma\rho( r_2+...|a_2,s_3)| a_1,s_2)$ by the reviewer). We have also further emphasized in Remark 2 and its footnote that the equivalence of the optimal solution of Markov risk measure and the risk-sensitive MDP holds because the optimal policy is deterministic, and it would fail if the optimal policy is no longer deterministic due to policy regularization.

Regarding the further concern of the reviewer that the definition of the value function of the risk-sensitive MDP is different from the dynamic risk measure $\rho(\sum_t\gamma^t r(s_t,a_t))$, we agree with the reviewer that these two notions modeled risk in a different manner and we have pointed it out in Appendix C. \textcolor{blue}{However, we would like to also clarify that even for Markov risk measures (i.e. $RPR = \rho(r_1+ \gamma\rho( r_2+...|a_2,s_3)| a_1,s_2)$) which considers $\rho$ to be a coherent risk measure with the scale invariance property (as defined in [70]), it is not equivalent to the term $\rho(\sum_t\gamma^t r(s_t,a_t))$. Even in [16], although in eq (2) of the paper it writes the risk measure as $\rho(\sum_t\gamma^t r(s_t,a_t))$, the true algorithm considers a dynamic risk measure that resembles the Markov risk measure (see eq(6) and (P1) in [16]). Yet we agree with the reviewer that since convex risk measures might not be scale-invariant, and thus the discounting factor $\gamma$ cannot be pulled inside/outside the risk measure, i.e. $r_1 + \gamma\rho(r_2) \neq r_1 + \rho(\gamma r_2)$.}

Once again, we express our gratitude to the reviewer for the time and effort put into reading the paper and the discussion. We are grateful for the reviewer's help in improving the clearness and rigorousness of the paper!

\paragraph{The third comment:} We would like to once again thank the reviewer for a thorough reading of our work! We have fixed the typos and changed the notation based on the reviewer's suggestions.





==> Response/Further_response_to_reviewer_2__round_2_.tex <==
\section{Further response to Reviewer 2 (Round 2)}

[In Response to 'Authors falsely claim that all convex risk measure are mixture quasiconcave'] We sincerely thank the reviewer for providing detailed clarifications to help resolve misunderstandings and miscommunications. We now have a better understanding of the source of the misunderstanding. We concur with the reviewer that for the statement 'the optimal solution of Markov risk measure and risk-sensitive MDP is the same' to be accurate, apart from showing that the optimal solution of risk-sensitive MDP is deterministic (which is proved in Theorem 2), we must also ensure that the optimal solution of the Markov risk measure is deterministic, which requires further assumption of mixture quasiconcavity. We have made revisions in Remark 2 as well as Appendix C. Here we quote the sentences from the revised Appendix C: 'Additionally, when the risk-measure $\sigma$ is mixture quasiconcave (c.f. Delage et al.), it can be shown that the optimal policy $\pi$ for the Markov risk measure can also be chosen as a deterministic policy; thus under this case the Markov risk measure and the risk-sensitive MDP obtain the same optimal value, i.e. $\Vmrm^\star = \tV^\star$. However, we would also like to emphasize that when adding policy regularization or that the risk measure $\sigma$ is not a mixture quasiconcave (e.g. mean semi-deviation), the optimal policy might no longer be a deterministic policy. In this setting, the optimal policy and optimal value of the Markov risk measure and the risk-sensitive MDP may not be the same.' 

Moreover, in case there is still unclearness or miscommunication since there are several ``equivalence'' being discussed, we would like to summarize a few points here, 1) The main equivalence theorem, Theorem 2, focuses on the equivalence of soft robust MDP and risk-sensitive MDP proposed in the paper. This theorem is accurate and it does not discuss the relationship of the optimal solution of Markov risk measure and risk-sensitive MDP. 2) Remark 2 and Appendix C discuss the relationship between the risk-sensitive MDP and Markov risk measure. We have revised the remark and appendix based on the discussion.

Again, we would like to express our regards and gratitude for the reviewer's time and effort in keeping the discussion and clarifying the confusion. We remain at the reviewer's disposal for any points requiring further discussion. 

[In Response to 'Further comments on limitation 2 and 3 of Theorem 2'] We apologize for misunderstanding the reviewer's comments. Previously, we interpreted the $\rho$ in $\rho(\sum_t^T\gamma^t r(s_t,a_t))$ in the reviewer's comment to be any type of coherent risk measures. After reading the reviewer's clarification, we agree with the reviewer that when $\rho_{0,T}$ is a time-consistent dynamic risk measure, it can be written as, $\rho_{0,T}(r_1, r_2, \ldots, r_T) = r_0(s_0, a_0) + \rho_0(\gamma r_1(s_1,a_1) + \dots + \rho_{T-1}(\gamma^T r_T(s_T, a_T)))=\rho_0(\rho_1(\ldots \rho_T(\sum_{t=0}^T \gamma^t r(s_t,a_t))\ldots))$, where $\rho_t, t=0,\ldots, T$ are one-step conditional risk measures as defined in [71] and satisfy the properties listed in the bottom of p.241.  Since we consider a different risk measure, it can no longer be written in this formulation. We have added a footnote in Remark 2 (highlighted in blue) to emphasize that our definition is different from the usual interpretation of the dynamic risk measures formulation of the risk-averse MDP problems. 

We would like to thank the reviewer again for the timely replies and active discussions. We hope that our paper revision as well as response clarifies the miscommunication and addresses the reviewer's questions and concerns. We are more than happy to engage in further discussion if there are any additional questions or concerns from the reviewer.
\section{Message to AC}

Thank you for handling our paper – we recognize that you are managing >10 submissions, and appreciate your dedication to ensuring a thorough review process! We were encouraged by the positive feedback received from several reviewers on the originality, technical quality, and theoretical grounding of our contributions to the field of risk-sensitive and robust RL.

In response to the reviewers' questions, we did our best to provide comprehensive and thoughtful answers. However, as of now, we have received responses from only one of the reviewers.

As the discussion period draws to a close, we would greatly appreciate it if you could remind the remaining reviewers to engage in the discussion. We would love to learn whether our responses have addressed their questions and if they have any additional suggestions that could help us further improve our paper. Thank you again for your time, understanding, and service to the community.

\section{Message to AC: Concerns and Clarifications Regarding Reviewer Feedback: Ambiguities in Terminology and Notations}
{\color{blue}
We would like to bring to your attention our concern regarding the terminology and notations discussed by reviewer RSEz. First of all, we deeply appreciate the reviewer's time and effort in his review and discussion. However, because of the limitation of the discussion format (i.e., typing comments/responses on chat window) and the complexity of terminologies and notations used in the literature on the subject of risk-measure and risk-aware decision-making, there are many ambiguities in the comments, as you can see from the back-and-forth discussion between the reviewer and us. 

As a concrete example, for the comments on 'Further comments on limitation 2 and 3 of Theorem 2' (add URL later), there is ambiguity in the interpretation of the equation: $\rho(\sum_t^T\gamma^t r(s_t,a_t)) = \rho(r_0(s_0, a_0) + \rho(\gamma r_1(s_1,a_1) + \dots + \rho(\gamma^T r_T(s_T, a_T)))$, We are uncertain whether the reviewer intends for the risk measures $\rho$ to be the same or different on both sides of the equation or if they are referring to different types of risk measures. In our response, we have endeavored to clarify this ambiguity, by drawing the exact equations from reference [71], to which the reviewer refers. we respond with a more precise formulation: $\rho_{0,T}(r_1, r_2, \ldots, r_T) = r_0(s_0, a_0) + \rho_0(\gamma r_1(s_1,a_1) + \dots + \rho_{T-1}(\gamma^T r_T(s_T, a_T)))=\rho_0(\rho_1(\cdots \rho_T(\sum_{t=0}^T \gamma^t r(s_t,a_t))))$ where $\rho_t$ are one-step conditional risk measures and $\rho_{0,T}$ is a composition of $\rho_t$'s.  As you can see, the risk measures on both sides need to be different to make the equation valid.   

We have put forth our best effort to interpret the reviewer's intended meaning, and there's a genuine concern that our interpretation might not entirely align with the reviewer's perspective. We are particularly worried that the reviewer could potentially misunderstand our argument, possibly leading to the perception that our response lacks rigor.

This message aims to emphasize our dedication to addressing the reviewer's comments with meticulous care and precision. We recognize the complexities of the discussion and are open to further clarification or guidance to ensure that our responses accurately convey the intended nuances. We sincerely hope our paper won't be penalized because of any inadvertent misinterpretation and miscommunication, and we remain committed to promptly addressing any concerns or providing additional clarifications as needed.

Your understanding and assistance in navigating this matter are greatly appreciated and invaluable to us.
}


%https://openreview.net/forum?id=dEz3ge8QSo&noteId=q9jkvjoFfT




==> Response/Reviewer_1.tex <==
\section{Response to Reviewer 1 (SuJM)}

We first sincerely thank the reviewer for carefully reading our paper and appreciating our contributions! We greatly appreciate the constructive suggestions and valuable questions from the reviewer. Prior to addressing the reviewer's comments, we would like to note that, due to the revision, reference/equation/remark numbers may differ. To maintain consistency with the reviewers' comments, *our responses will refer to the original version's reference/equation/theorem numbers unless explicitly specified otherwise.* Additionally, based on the insightful suggestion of Reviewer RSEz, we changed the term 'regularized robust MDP' to 'soft robust MDP'. We now address the questions and concerns raised by the reviewer as follows:

Response to the reviewer's concerns in the 'Weakness' section:

**[Comparison with [18] and [32]]** The reviewer raised the question of how our regularized MDP compares with the regularization term in [18]. We would like to first apologize for our misleading use of the term 'regularized robust MDP' (which is also pointed out by the third comment in the 'weakness' section of  Reviewer RSEz). As is also pointed out by Reviewer RSEz, the regularization in [18] and ours are different in the sense that the 'regularized MDP' in [18] considers regularization on the policy whereas in our setting the regularization is on the transition probability matrices. To avoid confusion, as suggested by Reviewer RSEz, we have changed 'regularized robust MDP' to 'soft robust MDP' in the revised version of the paper. Thank you for raising this valuable question! 

The reviewer also asked whether the same convex formulation in [32] applies to the regularized RMDPs (soft RMDPs). We are also interested in the same question and we actually had a brief discussion with one of the authors in [32]. Based on the discussion and our preliminary attempt, it might not be a trivial combination, and it is an interesting future direction to study how to leverage our formulation to get simplified convex formulations for (soft) RMDPs. In response to the reviewer's question of whether the gradient domination property is ensured by the above convex formulation, our current proof leverages the performance difference lemma and the key technique is inspired by the proof of gradient domination in standard MDP [2]. It would be an interesting research topic to study if the gradient domination property can be proved from the convex formulation perspective, but currently, it is unclear to us whether the convex formulation is directly related to the gradient domination property. 

**[Application of techniques in [101]]** The reviewer asked whether we could apply similar techniques in [101] (which we believe is the same reference as [44] in the original paper, we have updated the publisher info of [44] in the revised paper) by explicitly deriving the worst transition model $\widehat{P}^\pi$. We agree with the reviewer that in certain cases the worst-case probability transition model can indeed obtain an explicit/analytical form that can simplify the problem to a certain extent (e.g. entropy risk measure $\widehat{P}^\pi$ takes the form $\widehat{P}^\pi(s'|s,a)\propto P(s'|s,a)\exp(-\beta V^\pi(s'))$). We believe that in this case we could leverage techniques such as importance sampling or rejection sampling to make gradient estimation more amenable. However, based on our own calculation, the sample complexity analysis is more technically involved, which is one of the main reasons why we considered the RFZI algorithm instead of policy gradient algorithm for the sample-based learning setting and we left it as the next step of our research to study the performance of sample-based policy gradient for risk-sensitive MDPs and (soft) RMDPs. 

**[Motivation for the offline learning algorithm RFZI]** The reviewer questions the motivation of the offline learning algorithm in Section 5. The major motivation for Section 5 is to provide one sample-based learning algorithm for risk sensitivity MDPs and soft robust MDPs, since Section 4 only considers the learning algorithm with full information and studies the iteration complexity. Ideally, it would be better to design sample-based policy gradient methods.  However, as mentioned Remark 4, it is difficult to estimate the policy gradient by samples, which is why we first consider the RFZI algorithm which resembles policy iteration rather than policy gradient. The reason for considering the specific setting of offline learning algorithm with nonlinear function approximation is that, as mentioned in the introduction, it is a less-studied setting for RMDPs and we hope that our results could bring insights to make algorithm design and theoretical analysis easier for this less-studied scenario. We apologize for not explaining our motivations clearly and we hope that the above explanation clarifies the confusion of the reviewer. We have included part of the above discussion at the beginning of Section 5 and we are happy to have further discussions. We have also added more experimental results that study the robustness/risk-sensitive behavior of soft robust optimal policies and compare it with the robust optimal baseline (see Figure 4 and its related paragraphs in Appendix B).

**[Performance comparison with the RFQI algorithm in [61] and open questions in Section 5]** The reviewer suggests adding a comparison with the sample complexity bound of RFQI algorithm in [61]. We first thank the reviewer for the valuable suggestion. We agree with the reviewer that a comparison between the results of the two algorithms is necessary and we have added related discussions to the revised paper (highlighted in blue). Here we quote the discussion: 'We also compare our performance bound with the RFQI algorithm which considers a similar offline learning setting and obtains sample complexity of $O\left(\frac{\log(|\mathcal{F}||\mathcal{G}|)}{(\beta\epsilon)^2(1-\gamma)^6}\right)$, where $\beta$ in their setting is the diameter of the uncertainty set. Note that both results share the same dependency on the concentrability constant $C$ and the precision $\epsilon$. However, they have an additional term on the size of the space of the dual variable $\log |\mathcal{G}|$, whereas we have an additional exponential dependence term $O\left(e^{\frac{2\beta}{1-\gamma}}\right)$.' Yet we would also like to note that the two settings are not completely comparable as we consider different types of uncertainty sets and the algorithms are very different.

The reviewer also raised questions on the assumption and the theoretical bounds in Section 5. We address the questions as follows:

- *'Can Assumption 2 be avoided?'* We would like to refer the reader to Remark 6 where we provide a detailed discussion on Assumption 2. In particular, Assumption 2 is adapted from the
corresponding notions defined for the standard MDP setting [11], where they also demonstrate the necessity of this assumption for standard RL with function approximation. However, for the risk-sensitive and soft robust MDP settings, we currently don't have theoretical results to verify the necessity of Assumption 2. It would be an interesting
open question whether Assumption 2 is also necessary.


- *'How to empirically select the penalty factor and shrink the performance gap?'* Remark 7 provides a brief discussion on the choice of $\beta$ where we quote as follows:  the term $\beta^{-1}e^{\frac{\beta}{1-\gamma}}$ first decreases and then increases with $\beta$ as it goes from $0$ to $+\infty$, suggesting that the hyperparameter $\beta$ also affects the learning difficulty of the problem. The choice of $\beta$ should be neither too large nor too small, ideally on the same scale with $1-\gamma$. We would also love to add further discussions if the above discussion is not detailed enough!

- *'Is the exponential dependence a proof artifact or is it intrinsic to the problem?'* Thanks for the question! It is still unclear to us whether it is a proof artifact or intrinsic in our setting, however, there are results under similar settings that suggest this exponential dependency on parameter $\beta$ and the effective length $\frac{1}{1-\gamma}$ is fundamental (e.g. Theorem 3 in [23]). We have added the above discussion to Remark 6 in the revised paper (previously Remark 7 in the original version, highlighted in blue).

 Response to the reviewer's questions in the 'Questions' section:

**[Discussion between terms 'unknown model', 'model-based', 'model-free']** We apologize for the confusion. By 'unknown model' we refer to the setting where the nominal probability transition $P$ model is unknown. Both 'model-based' and 'model-free' methods belong to the setting with 'unknown model'. Although 'Model-based' methods don't have knowledge about the nominal probability transition, they generally keep an empirical estimate of the nominal model $P^{\textup{est}}$ and the algorithms rely heavily on the estimated model $P^{\textup{est}}$. However, in comparison 'model-free' algorithms don't require this empirical estimation step and thus might be more suitable for large-scale problems. We categorize [48] as model-based (the algorithm requires an empirical estimation $\hat{P}_k$ as an input). Our algorithm only requires learning the Z-function and does not rely on an estimated model and thus belongs to the 'model-free' category. We have added the above discussion as a footnote in the revised paper. Additionally, we would also like to clarify that for RMDP, people generally refer 'known/unknown model' as the nominal model rather than the uncertainty set. In the RMDP setting, the uncertainty set is generally assumed to be known and pre-given as an algorithm input. Based on our understanding of [48], we believe they still require knowledge of the uncertainty set but don't require knowledge of the nominal model.

**[Clarification of Remark 1]** We apologize for the imprecise language and thank the reviewer for pointing out potential improvements. We have revised the sentence based on the suggestion of the reviewer. Regarding the relationship between 'model-based' and 'model-free' learning, as mentioned in the previous paragraph, for RMDP, people generally refer 'known/unknown model' as the nominal model rather than the uncertainty set, so it is not directly related.

**[Relationship between Theorem 1 and Fenchel conjugate]** The reviewer's understanding is correct. In the finite-dimensional case, the penalty function $D$ is the Fenchel conjugate of $\sigma$. We have added a short remark in our revised paper to make it clearer. We would also like to clarify that Theorem 1 is not an original contribution of our work; instead, we reference this theorem from classical literature [27], as it forms the foundation for the subsequent content of our paper.

**[Intuitive explanation of the difference of the value function for risk-sensitive MDP and the Markov risk measure]** Thanks for the question. Due to the space limit, the more detailed explanation and comparison of the risk-sensitive MDP and the Markov risk measure was deferred in Appendix C. Intuitively speaking, the Markov risk measure also takes the risk generated by the randomness of the policy into account whereas our definition treats the randomness from the policy in a risk-neutral manner and only considers risk from the uncertainty of the transition probability. This intuitively explains why the two notions are equivalent for deterministic policies but not for stochastic policies. We have added the above intuitive explanation to Appendix C in the revised paper (highlighted in blue). We would also like to emphasize that our definition of risk-sensitive MDPs has its own benefits. It results in a cleaner equivalence with (soft) RMDPs and better convergence property compared with directly optimizing the Markov risk measure, which is known to be possibly non-gradient dominant (c.f. [36]).  Consequently, our results provide an alternative approach for the efficient optimization of the Markov risk measure, despite modeling risk in a different manner.

**[Suggested corrections]** We extend our sincere gratitude to the reviewer for carefully going through the paper and pointing out typos, inaccurate reference information, and other corrections! We have fixed the typos and references, deleted unnecessary content and remarks, and revised our paper based on the suggestions from the reviewer. We have also provided additional elaboration in the introduction, specifically addressing the motivation behind our offline learning algorithm and how it overcomes the shortcomings highlighted earlier. Given the richness of the field of robust and risk-sensitive learning, we regret that we could not include all the literature in the main text. We still kindly refer the reviewer to Appendix A for a more comprehensive comparison with prior works.

We would also like to note that the publisher information is not updated for a few papers in the reference because they are not officially published yet based on our literature search. We would be happy to make further updates on the references if there are any further questions or suggestions! 

With regard to the reviewer's suggestion of putting the definition of risk-sensitive MDP into Section 3, we apologize that, after careful consideration, we still decide to keep the original structure. We believe that maintaining Section 2 as a self-contained section with all the preliminaries logically aligns with the overall flow of the paper. We are open to further discussion regarding the paper's structure and appreciate the reviewer's input on this matter.


Once again, we sincerely thank the reviewer for dedicating time and effort to a thorough review of our paper. We hope that our response could clarify the questions and concerns of the reviewer and we are happy to address any other questions the reviewer has!

==> Response/Reviewer_2.tex <==
\section{Response to Reviewer 2 (RSEz)}

We sincerely thank the reviewer for carefully reading our paper, acknowledging our contributions, and giving insightful and critical feedback! Prior to addressing the reviewer's comments, we would like to note that, due to the revision, reference/equation/remark numbers may differ. To maintain consistency with the reviewers' comments, *our responses will refer to the original version's reference/equation/theorem numbers unless explicitly specified otherwise.* We now address the concerns raised by the reviewer in the 'Weakness' section as follows:

**[Term of 'regularized robust MDP']** The reviewer pointed out that the term 'regularized robust MDP' might be misleading. We sincerely thank the reviewer for presenting more accurate alternatives and providing related references. After reading the references, we fully agree with the reviewer that 'soft robust MDP' indeed encapsulates the intended concept more accurately. We have changed the name of the term to `soft RMDP' and added related references in our revised paper. We will use soft RMDP in the response as well.

**[Limitation of Theorem 2]** The reviewer has pointed out several limitations of Theorem 2, which we summarize below: 1. The equivalence only holds for convex risk measures (referred to as 'quasi-concave/mixture quasi-concave' by the reviewer) and does not generalize to other risk metrics such as mean (semi-)deviation
and mean (semi-)moment measures in Delage et al. (2019) ; 2. The equivalence would fail if policy regularization is added to the objective function, in which case the optimal policy might be stochastic. 3. The risk-sensitive MDP underestimates the risk caused by the stochasticity generated by the policy. 

We now address the reviewer's comments point by point:

For point 1, we agree with the reviewer that the equivalence no longer holds if we consider other risk metrics other than convex risk measures. However, we would like to note that the convex risk measure is an important risk metric and is commonly used in finance and operations research. Consequently, our findings establish a meaningful foundation for exploring risk-sensitive sequential decision-making, albeit within the confines of convex risk measures. An intriguing avenue for future research would involve investigating reinforcement learning or sequential decision-making in the context of diverse risk metrics.
However, given the distinct properties of risk metrics like semi-deviation and semi-moments in comparison to convex risk measures, different theoretical tools may be necessary, which poses challenges to the analysis, and unfortunately falls outside the current scope of this paper.

For point 2, we would like to clarify that this is actually not the case: the equivalence between the value functions of risk-sensitive MDPs $\tV^\pi$ and soft RMDPs $\oV^\pi$ will still hold under most classical policy regularization methods (e.g. entropy regularization). Note that Theorem 2 holds not just for deterministic policies, but also for stochastic policies. For a policy $\pi$, adding regularization only requires changing the reward function $r(s,a)$ to be $r^\pi(s,a) = r(s,a) + \mathcal{R}(\pi(\cdot|s))$, where $\mathcal{R}$ is the policy regularizer. In this setting, the proof of Theorem 2 can still carry through naturally. We have added the above discussion as a footnote in the revised paper (highlighted in blue).

For point 3, we would like to first thank the reviewer for the insightful comment! The reviewer is correct that the proposed risk-sensitive MDP focuses on the risk induced by the uncertainty set but does not consider the risk caused by the stochastic policy. However, we would like to emphasize that this different definition of risk has its advantages. Although the formulation of risk-sensitive MDP differs from the standard definition of dynamic risk (Pichlet et al. 2021), which we believe is the same definition as the Markov risk measure [67], they both yield identical optimal values and optimal policies (see Remark 2 and Appendix C for more detail). Further, this different formulation results in a cleaner equivalence with (soft) RMDPs and better convergence property compared with directly optimizing the Markov risk measure, which is known to be possibly non-gradient dominant (c.f. [36])  Consequently, our results provide an alternative approach for the efficient optimization of the Markov risk measure, despite modeling risk in a different manner. However, we also agree with the reviewer that optimizing the Markov risk measure with policy regularization would potentially result in a different optimal solution compared with the solution of our risk-sensitive MDP with policy regularization.


**[Novelty of Results]** The reviewer pointed out that some of the results in this paper follow closely from existing work. Here we respectfully reference the comments from the reviewer and aim to address these observations by clarifying our contributions and novelty in comparison to prior studies.

*'Theorem 1 comes from [27]. The equivalence between soft robust optimization and convex risk measure is already established in Ben-Tal et al. (2010). It is therefore no surprise that the result in Theorem 2 would hold.'* We would like to first clarify that the dual representation theorem (Theorem 1) is not claimed to be a contribution of our work; instead, we reference this theorem from classical literature, as it forms the foundation for the subsequent content of our paper. Regarding the significance of Theorem 2, we agree with the reviewer that the proof intuition follows from Theorem 1 and it might not be surprising for readers who are familiar with both dynamic programming and risk measures. However, we would like to note that it is not a direct or trivial generalization of Theorem 1, as it considers the MDP setting, which has a sequential structure that is more complicated than the static setting considered in Theorem 1. The proof (detailed in Appendix E) also requires a careful combination of dynamic programming with the dual representation theorem. As far as we know, although there are many works that discuss the relationship between robustness and risk-sensitivity (see Appendix A in our paper for more detail), there's no result that explicitly states the exact equivalence between (soft) RMPD and risk-sensitive MDP. We believe that Theorem 2, therefore, remains a distinctive and interesting contribution with its own merits.

*'Theorem 3, Lemma 2, and Theorem 4 extend the result of [85] from robust MDP to the slightly more general regularized/soft robust MDP.'* Thanks for the comment and for directing us to the most related literature [85]. Here we briefly list the major differences between our paper and [85]. Firstly, we obtain an explicit analytical form of the policy gradient in Theorem 3, whereas in [85], they consider the Moreau envelope of the value function and it is implicitly computed through a double-loop manner. This immediately leads to the next two differences--different algorithm designs and different theoretical bounds. [85] needs to consider a modified policy gradient with a double-loop, whereas our algorithm removes the double-loop and studies policy gradient without modification. Given the simpler algorithm design, our iteration complexity also has a better dependency on the size of the state and action spaces $|\cS|,|\cA|$ as well as the distributional shift factor $M$ (denoted as $D$ in [85]).
However, we also acknowledge that [85] has considered settings more general than our paper, e.g. it also takes the $s$-rectangularity setting into consideration. It would be an interesting next step to see if we could  combine insights from both works to have more general and improved results.

*'Section 5 proposes an algorithm that resembles the approach presented in [24] although I am not aware of a sample complexity result for that class of algorithm.'* We express our gratitude to the reviewer for recognizing the novelty of our sample complexity result. We would like to first clarify that the objective function considered in [24], namely the exponential utility, differs from our objective function (see more elaboration in the third paragraph in 'Other related works' in Appendix A). Additionally, the learning settings as well as the algorithms are different. [24] considers online learning in the tabular setting and the algorithm is based on Q-learning, whereas we consider offline learning with function approximation and the algorithm resembles policy iteration type of algorithms. 

**[Proof to verify]** The reviewer suggests a more detailed verification of equation (25) on page 34. We have already added more details for (25) to the revised paper (highlighted in blue on page 31 in the revised version). However, we find that equation (25) is on page 27 instead of page 34, so we are uncertain if we've tackled the right equation that the reviewer questioned. We would be happy to discuss the technical proofs if there are still equations that are unclear.

**[Typos/clarifications]** We sincerely thank the reviewer for carefully going through the paper and pointing out typos and other possible corrections and improvements. We have incorporated the reviewer's suggestions into the revised version of the paper. (For the notation $\cT^\star, \cT^\pi$, because it is originally defined as the Bellman operator for the risk-sensitive MDP instead of soft RMDP, we decide to keep the original notation $\cT$ rather than $\overline\cT$ as suggested by the reviewer.) It seems that the page numbers referenced by the reviewer might be slightly inaccurate. We remain open to making additional revisions if our current modifications do not align with the reviewer's intended recommendations.

Once again, we are grateful for the reviewer's insightful comments and constructive suggestions! We remain at the reviewer's disposal for any further inquiries or points requiring additional discussion. Your valuable input is greatly appreciated.

==> Response/Reviewer_3.tex <==
\section{Response to Reviewer 3 (BzBp)}
We sincerely thank the reviewer for appreciating the contribution of our work! Prior to addressing the reviewer's comments, we would like to note that, due to the revision, reference/equation/theorem numbers may differ. To maintain consistency with the reviewers' comments, *our responses will refer to the original version's reference/equation/theorem numbers, unless explicitly specified otherwise.* Additionally, based on the insightful suggestion of Reviewer RSEz, we changed the term 'regularized robust MDP' to 'soft robust MDP'.

We now address the reviewer's questions as follows:

*'Could the authors provide some examples where theorem 2 is applied to establish the equivalence between some popular regularized RMDPs and risk-sensitve MDPs?'*

One example for the soft RMDPs and risk-sensitive MDPs is the soft-KL RMDP, which is equivalent to the risk-sensitive MDP with entropy regularizer. This example is discussed in more detail in Section 5 of the paper.

Another example can be the risk-sensitive MDP with Conditional value at risk (CVaR, see Example 2 in the original version). Leveraging Theorem 2, it is equivalent to the RMDP with uncertainty set $\{\frac{\widehat{P}(s'|s,a)}{P(s'|s,a)}\le {\alpha^{-1}}, \forall ~s',s\in\cS, a\in\cA \}$ 

*'In section 2, the authors introduce convex risk measures, where there is only one input in the measure $\sigma$ in (5) and (6), while there are two in examples 1 and 2. Could the authors explain what is the difference between these two $\sigma$'s?'*

Thanks for the question! In the paper, we provide an explanation after Theorem 1 that clarifies the two inputs in the risk measure $\sigma$ as well as the penalty function $D$, which we quote as follows: 'In most cases, the convex risk measure $\sigma(V)$ can be interpreted as the risk associated with a random variable that takes on values $V(s)$ where $s$ is drawn from some distribution $s\!\sim\!\mu$. Consequently, most commonly used risk measures are typically associated with an underlying probability distribution $\mu\!\in\!\Delta^{|\cS|}$ (e.g., Examples 1 and 2). This paper focuses on this type of risk measures and thus we use $\sigma(\mu,\cdot)$ to denote the risk measure, where the additional variable $\mu$ indicates the associated probability distribution.  %The larger $\sigma(\mu,V)$ is, the larger the risk is. 
Correspondingly, we denote the penalty term $D(\hat{\mu})$ of $\sigma(\mu,\cdot)$ in the dual representation theorem as $D(\hat{\mu},\mu)$.' We hope that this answers the reviewer's question and we are happy to further discuss if there are any parts that remain ambiguous.

*'What is "direct parameterization"?'* and *'About the feasible region 
$\cX$ of $\theta$ : why it is of dimension $SA$ 
? And why each subvector $\theta_s$ should be in the probability simplex?'*

Direct parameterization is one of the most commonly considered approaches to parameterize a policy in theoretical RL (c.f. [2]). As we have stated before Corollary 1, 'for direct parameterization, the parameter $\theta_{s,a}$ directly represents the probability of choosing action $a$ at state $s$, i.e., $\theta_{s,a} = \pi_\theta(a|s)$.' We have also added some standard references for direct parameterization in the same paragraph. 

Given this definition of direct parameterization, $\theta$ is of dimension $SA$ because for each $s$ and $a$, there's a corresponding entry $\theta_{s,a}$ that represents $\theta_{s,a} = \pi_\theta(a|s)$. Further, the subvect $\theta_{s}$ represents $\theta_s = \pi_\theta(\cdot|s)$ which lies in the probability simplex. We hope that the above response answers the reviewer's question!

*'Is the right-hand side of (15) independent of the initial distribution $\rho$?'*

Thank you for reading into the technical details. The right-hand side of (15) is actually dependent on the initial distribution $\rho$ because the discounted state visitation distribution $d^{\pi_\theta, \hP\theta}$ (defined at the end of Section 2) is dependent on $\rho$.


*Assumption 1, typo in the first sentence.* Thank you for pointing out the typo! We have corrected it in the revised paper.

*Assumption 3, what is the norm with subscript "$2,\mu$"?*

Thank you very much for the question! We recognized that we didn't give a formal definition of $\|\cdot\|_{2,\mu}$ in the original version. For any function $f:\cS\times\cA\to \bR$, state-action distribution $\mu\in\Delta(\cS\times\cA)$, the $\mu$-weighted 2-norm of $f$ is defined as $\|f\|_{2,\mu} = \left(\bE_{s,a\sim\mu}f(s, a)^2\right)^{1/2}$. We have added the above definition to the preliminary section of the paper (highlighted in blue). We sincerely appreciate your contribution in highlighting this particular omission.

In conclusion, we express our sincere gratitude to the reviewer for the constructive comments and feedback. We are happy to have further discussions if there are any other questions!

==> Response/Reviewer_4.tex <==
\section{Response to Reviewer 4 (KqgB)}
We sincerely thank the reviewer for a thorough examination of our paper and for giving critical and valuable feedback! Prior to addressing the reviewer's comments, we would like to note that, due to the revision, reference/equation/theorem numbers may differ. To maintain consistency with the reviewers' comments, *our responses will refer to the original version's reference/equation/theorem numbers, unless explicitly specified otherwise.* Additionally, based on the insightful suggestion of Reviewer RSEz, we changed the term 'regularized robust MDP' to 'soft robust MDP'.

We now address the reviewer's questions and concerns as follows:

Weakness:

*'The authors fail to explicitly differentiate between stationary and non-stationary policies, as well as between stochastic and deterministic policies. While Equations (1) and (2) suggest that the authors are considering a robust MDP with a non-stationary and deterministic policy, Equations (7) and (8) indicate a stationary and stochastic policy for the risk-sensitive MDP. A similar inconsistency is observed in the transition kernel: while the robust MDP seems to consider the worst-case transition kernel for each time horizon (as evidenced by the decision variables in the infimum problem of Equations (1) and (2)), the risk-sensitive MDP presumes the existence of a transition kernel that is independent of time.'*

We sincerely apologize for the confusion. However, we would like to clarify that our definitions and derivations are technically correct. For the sake of generality, in Eq (1),(2) and (3) of the definition of robust MDP, we allow the policy as well as the transition kernel to be non-stationary. However, Theorem 2 points out that the sup-inf solution of equation (1)(2)(3) can be obtained by stationary policies and stationary transition kernels (Eq (11),(12)). Thus it is sufficient to restrict the later discussions to stationary policies and transition kernels, which is why our definition of value functions (e.g. Eq (4) and (7)) are only defined for stationary policies. Regarding the reviewers' concern of the differentiation between deterministic policies and stochastic policies, we apologize for our inaccurate notation which causes this confusion. The optimal value function is actually defined as the supremum over all possible policies which can be potentially stochastic, non-stationary and non-Markovian. However, the optimal solution can be obtained by a deterministic stationary Markov policy. We have updated our definition of equation (1)(2)(3) and added the above discussion as a footnote in the revised paper (highlighted in blue).

We would also like to note that our definition and analysis resemble the standard argument for risk-neutral MDP counterparts, where the original definition of the optimal value function considers taking the supremum over all possible non-stationary, even non-Markovian policies, yet it is shown that the optimal policy can be obtained by a stationary deterministic Markov policy. We hope that the above discussion clarifies the reviewer's confusion and we are open to further discussions if there are any follow-up questions from the reviewer. 

Questions:

*'Within the framework of risk-sensitive MDP, the value function for a given policy $\pi$, denoted as $\widetilde{V}^\pi(s)$, is defined by equation (7). The optimal value function, $\widetilde{V}^\star$
, is defined as $\max_\pi \widetilde{V}^\pi(s)$. Could the authors elucidate how $\widetilde{V}^\star$ satisfies the equation (9)?'*

Thanks for reading carefully into the technical details in the paper! We would like to clarify that the definition of the optimal value function $\tV^\star$ is actually initially defined as Eq (9) and then in Theorem 2, we show that $\tV^\star(s) = \max_{\pi} \tV^\pi(s)$, i.e. the optimal value function can be achieved by a Markov policy, which is proved in Appendix E at the beginning of page 24, where it shows that there exists a $\pi^\star$, such that $\tV^\star = \tV^{\pi^\star}$.


*'As noted in remark 7, the sample complexity of the proposed algorithm appears less favorable than that detailed in reference [11], assuming that there is no function approximation error in the authors' approach, $\epsilon_c = 0$. What then are the advantages of the corresponding RFZI algorithm? Furthermore, given the resemblance between Equations (7) and (9) and the traditional Bellman equation, and considering that the operators are proven contractions, is it feasible for the authors to employ value iteration or policy iteration to resolve the MDP? Such methods should theoretically exhibit rapid (geometric) convergence and remain unaffected by unknown exact gradients present in policy gradient methods.'*

Regarding the reviewer's question about the advantage of RFZI over reference [11], we would like to clarify that reference [11] considers the standard non-robust/risk-neutral RL, which is a different and possibly simpler setting compared with the robust/risk-sensitive setting considered in this paper. Based on the suggestion by other reviewers, we also added a discussion that compares our paper with an offline learning algorithm for RMDP [61] which is a more fair comparison (see Remark 6 in the revised paper (previously Remark 7 in the original version) and the response to Reviewer SuJM [Performance comparison with RFQI algorithm in [61]] for more details).

Regarding the reviewer's question of employing value iteration or policy iteration to resolve the MDP, our RFZI algorithm actually resembles policy iteration. In specific, the motivation of the algorithm is to solve the optimal Q function by solving the Bellman equation $Q^\star=\Tq Q^\star$. However, $\Tq$ involves a term $\log\bE_{s'\sim\Psa}$ which is hard to approximate with empirical estimation. Thus, instead of directly solving $Q^*$ using $Q^\star=\Tq Q^\star$, we introduce the Z-functions as auxilliary variables and solve the approximated fix point equation for $Z$. And the contraction of the Bellman operator is also reflected in our theoretical bound, where the first part $\frac{2\gamma^K}{(1-\gamma)^2}$ captures the effect of $\gamma$-contraction of the Bellman operators.

*'At the end of remark 7, the authors claim that the choice of $\beta$ should not be too large or too small, and would be better if it is on the same scale with $1-\gamma$. $\beta$ 
 is the radius of the ambiguity set related to the transition kernel and $\gamma$ is the discounted factor. It seems unconventional to determine the ambiguity set's radius based solely on the discount factor. Could this choice be elaborated upon?' *
 
 Thank you for the valuable question. We would first like to clarify that $\beta$ serves as an indicator of the penalty strength of the deviation of $\hat{P}$ from $P$ instead of the radius of the ambiguity set. The smaller $\beta$
is, the larger the penalty strength. Thus it can be expected that the sample complexity bound depends on both $\beta$ and $\gamma$, as they together determine the landscape of the problem. We concur with the reviewer that it looks counter-intuitive at first glance that the choice of $\beta$ should be 'on the same scale with $1-\gamma$'. The main reason lies in the exponential dependency term $O\left(e^{\frac{\beta}{1-\gamma}}\right)$ that shows up in the upper bound. It is still unclear to us whether it is a proof artifact or intrinsic in our setting, however, there are results under similar settings that suggest this exponential dependency is fundamental (e.g. Theorem 3 in [23]). Numerical evidence also suggests that large $\beta$ would affect the learning stability and typically people choose the hyper-parameter $\beta$ to be roughly on the same scale as $1-\gamma$ (e.g. [55]). Additionally, we emphasize that the choice of $\beta$ doesn't depend solely on $\gamma$ and might be related to the specific structure of the MDP, hence validation and hyperparameter tuning is still necessary for choosing $\beta$.  We have added parts of the above discussion in Remark 6 in the revised paper (previously Remark 7 in the original version).

*'In 'E.2 Proof of theorem 2 (infinite horizon case)' on page 23, the authors claim that it is not hard to show 
    $\lim_{h\to+\infty}\overline{V}_{0:h}^\star =\overline{V}^\star, \lim_{h\to+\infty}\overline{V}_{0:h}^\pi = \overline{V}^\pi$. This assertion doesn't immediately resonate with me. Would it be possible to furnish a detailed proof for this claim? Subsequent statements, $\overline{V}^\star = \mathcal{T}^\star\overline{V}^\star $ and $\overline{V}^\pi = \mathcal{T}^\pi \overline{V}^\pi $ also require clarification.'*
    
Thanks again for reading carefully into the proofs! We have added a more detailed proof in the corresponding locations (highlighted in blue). The key step is to show that $|\overline{V}^\pi(s) - \overline{V}_{0:h}^\pi(s)| |\overline{V}^\star(s) - \overline{V}_{0:h}^\star(s)| \le \frac{\gamma^h}{1-\gamma}$. And then by leveraging the continuous property of $\mathcal{T}^\pi, \mathcal{T}^\star$, we get $\overline{V}^\star = \mathcal{T}^\star\overline{V}^\star, \overline{V}^\pi = \mathcal{T}^\pi \overline{V}^\pi $.

Once again, we extend our sincere gratitude to the reviewer for the insightful comments and questions. We hope that our response clarifies the reviewer's concerns and we are more than willing to engage in further discussion to address any additional questions or concerns the reviewer may have.




==> Response/runyu_TODO_list.tex <==
\section{Runyu's TODO list for paper revision}
\begin{itemize}
    %\item Direct parameterization, cite standard references
    \item Performance difference Lemma
    \item Figure 4 add contents and elaboration
\end{itemize}

% Reviewer 1's comment lists:


% I do not see the utility of the paragraph on finite-horizon (referred to as (*) in the following item), to explain the fixed point equation (7). This is standard in MDPs and would save some valuable space that seems to be missing in this work. Instead, it would be useful to briefly mention the properties of the operator (7) -- monotonicity, sub-distributivity, contraction -- and how they follow from those of the convex risk measure 
% .

% In general, I think that the authors could and should shrink some parts of the text to better motivate their approach, and defer some explanation details of their method to the appendix. For example, Ex. 2 could be removed/put into the appendix, as it is not further used in the paper (as opposed to Ex. 1); the paragraph (*) could be removed completely. As such, instead of declaring "Due to space limit, we defer a detailed literature review and numerical simulations to the appendix", the authors could provide more synthetic exposition of their method, but detail more on its positioning w.r.t. previous works. Please see my questions in that respect.

% In the same spirit of saving space, the "other notations" paragraph at the end of Sec. 2 could be written inline and deferred to the "MDPs" paragraph at the beginning of Sec. 2; 

% Remarks may be written as regular text.

%Reviewer 2:

%Page 5, in the middle "Risk-Sensitive MDPs" misspell "Senstive" Page 5, the line above equation (7), misspell "valule" Page 8, Assumption 1, "For any policy pi and " missing P Page 25, paragraph under section C, last part, repeat expression "is defined as is defined as” Page 26, the notation would be clearer if the two “T^\pi” and “T^*” operators were denoted as “bar T^\pi” and “bar T^*” since they are defined in terms of the robust MDP Page 26, last part of Proof of Lemma1, "Lemma 1 is an immediate corollary of Lemma 8", it should be Lemma 3. "\tilde V and \tilde V^\star in (4) and (3)", it should be (7) and (9). Page 27, in Lemma 4, the definition of \mathcal{T}^* should be clarified. Page 28, In the proof of Lemma 4, \mathbb{E}{s_1\sim \hat{P}{0} should have a uniform expression as the passages above and below, i.e., \mathbb{E}{s_1\sim \hat{P}{0;s_0,a_0}. In line 4, there is a missing bracket in the last equation. Page 32, in Part G, the performance Difference Lemma [40] should be stated separately, as it has been applied a lot of times in the proofs. It is better to illustrate how this lemma is applied to this specific case.





==> Sections/Intro-09-16.tex <==
\section{Introduction}
Risk-sensitive decison making is important not only because it could capture take the level of uncertainty and associated risks into consideration, but also
% Maybe motivating it through risk-sensitive MDP. Risk is important not only because it could capture risk for uncertaintly, but also there's a elegant equivalence between risk and robustness.

% This elegant equivalence can extend to the MDP setting, as shown by ..., which introduced the Markov risk measure and  build the equivalence between minimizing the Markov risk measure and solving a min-max Markov control problem. Following this trial of working, a lot of learning algorithms are designed (cite temporal difference for Markov risk measures and policy gradient)

% However, learning for Markov risk measures encountered certain difficulties. Non-gradient dominance,  Also for temporal different learning (No sample complexity guarantees). Additionally, we would like to note that the equivalence is also not exact equivalence to RMDPs

The relationship between robustness and risk for MDPs is well-studied. \cite{ruszczynski2010risk,shen2013risk, BAUERLE2022953,bauerle2022distributionally} build the equivalence between minimizing the Markov risk measure and solving a min-max Markov control problem. However, the uncertainty set (or risk envelope) for the min-max would change with the policy implemented, especially when stochastic policies are considered (see Remark \ref{rmk:difference-with-Markov-risk-measure}), which is different from the standard formulation of RMDPs, where the uncertainty sets is not related to the policy. \citep{osogami2012robustness} obtains stronger results of equivalence to RMDP yet only for certain type of risk measures such as Conditional Value at Risk (CVaR).

There are many previous works focusing on applying policy gradient-based algorithm for risk-sensitive/robust learning \cite{tamar2012policy, tamar2015policy, tamar2017sequential, huang2021convergence, yu2023global, jaimungal2022robust, coache2023reinforcement, wang2022convergence,wang2022policy,kumar2023policy,li2023policy}. However, most of the works lack theoretical guarantees on the global convergence of these gradient-based algorithms \cite{tamar2012policy, tamar2015policy, tamar2017sequential,jaimungal2022robust, coache2023reinforcement}. \citet{huang2021convergence} give negative results showing that Markov risk measures are not gradient-dominant. \citet{yu2023global} prove global convergence for one specific type of risk measure - expected conditional risk measures (ECRMs).

 We would like to emphasize that, although taken a similar recursive form, the value function for our risk-sensitive MDP is actually \emph{different} from the Markov risk measure considered in most previous literature (e.g. \citep{ruszczynski2006conditional,huang2021convergence,tamar2015policy,tamar2017sequential}, detailed elaboration in Remark \ref{rmk:difference-with-Markov-risk-measure}). This slightly different definition of risk-sensitive MDP enables \emph{a stronger and more general equivalence with (reguarized) RMDP, a cleaner policy gradient theorem and better convergence property (gradient domination) as well as simpler offline RL algorithm design.

==> Sections/Intro-09-17.tex <==
\vspace{-10pt}
\section{Introduction}
\vspace{-5pt}
Decision-making in the face of uncertainty is a fundamental challenge across various fields such as finance \citep{follmer2016stochastic,sriboonchita2009stochastic}, engineering \citep{khan2016dynamic,shahidehpour2003market}, and robotics \citep{thrun2000probabilistic} etc. In these domains, decisions carry consequences that depend not only on expected rewards but also on the level of uncertainty or associated risks. Addressing this challenge necessitates approaches such as robust, or risk-sensitive decision-making. These approaches explicitly incorporate uncertainty and aim to find policies that perform well across a spectrum of scenarios or effectively balance the tension between expected gains and potential risks. 

%In the static setting \Lina{it is unclear what "static'' means here because the previous paragraph didn't say anything static, dynamic.}, 

When the uncertainty only involves a static random variable. it is well-known that there exists an elegant equivalence between risk and robustness. The notion of coherent risk measure was first proposed and studied in financial systems \citep{artzner1999coherent,delbaen2002coherent,rockafellar2000optimization}, where the relationship to robustness is also established by characterizing risk measures as the infimum of expected shortfall over a set of probability measures (risk envelope). The notion of coherent risk measure is further extended to convex risk measures that can capture a broader class of risk evaluation functions \citep{follmer2002convex,ruszczynski2006optimization,follmer2002robust}. 

Then the conditional/dynamic risk measures are introduced to generalize the risk for a static random variable to a stochastic process with a sequence of random variables \citep{artzner2007coherent,cheridito2006dynamic,follmer2006convex,detlefsen2005conditional,riedel2004dynamic,ruszczynski2006conditional}. \citet{ruszczynski2010risk} further applies the notion of conditional coherent risk measure to MDPs and introduced the Markov risk measure. However, the equivalence between Markov risk measure and robust planning is not as straight-forward as in the static setting. In particular, \cite{ruszczynski2010risk,shen2013risk, BAUERLE2022953,bauerle2022distributionally} build the equivalence between minimizing the Markov risk measure and solving a min-max Markov control problem, yet the uncertainty set (or risk envelope) for the min-max would change with the policy implemented, especially when stochastic policies are considered (see Remark \ref{rmk:difference-with-Markov-risk-measure}), which is different from the standard formulation of RMDPs (cite??)\Lina{Runyu, robust MDP has not been introduced yet. You would need to revise this paragraph to smoothly introduce robust MDP somewhere}, where the uncertainty sets are not related to the policy. \cite{osogami2012robustness} obtains stronger results of equivalence to RMDP yet only for certain types of risk measures such as Conditional Value at Risk (CVaR).

The policy-dependent risk envelope for Markov risk measures also makes optimizing it \Lina{would like to change "optimizing it". It is unclear what ``it'', especially you have "measures''}harder in the reinforcement learning (RL) settings. \citet{huang2021convergence} demonstrate that Markov risk measures can be not gradient-dominant even in the tabular setting with direct parameterization, which forms a sharp contrast with the gradient domination result in the standard MDP \citep{agarwal2020}. This suggests that policy gradient algorithms are not guaranteed to find global optimum even in this simple and full information setting. Further, the sample complexity seems to be harder to obtain.
There is a series of works dedicated to optimizing the Markov risk measure under the RL setting \citep{ccavucs2014computational,shen2014risk,kose2021risk}, yet only asymptotic convergence results are shown.

The aforementioned challenges motivate us to study whether we could propose another slightly different risk formulation that captures the risk in a similar fashion as Markov risk measures but provides a stronger and more general equivalence with RMDP, better convergence property (such as gradient domination), as well as facilitates the design of learning algorithms with provable guarantees.

\Lina{I see the current flow almost dowmplay ``robust MDP''. or at least Robust MDP was not discussed well enough... }
% ---------------------------------------------------


\noindent\textbf{Our Contributions:}  
In this paper, we study the iteration and sample complexity of reinforcement learning for a regularized RMDP problem, which subsumes RMDP as a special case. To gain a better understanding of the problem, we begin by introducing the risk-sensitive MDP, whose definition incorporates the concept of convex risk measures, and establishing the equivalence between these two problems (Theorem \ref{theorem:dual-representation}). We would like to emphasize that, although it takes a similar recursive form, the value function for our risk-sensitive MDP is actually \emph{different} from the Markov risk measure considered in most previous literature (e.g. \citep{ruszczynski2006conditional,huang2021convergence,tamar2015policy,tamar2017sequential}, detailed elaboration in Remark \ref{rmk:difference-with-Markov-risk-measure}). This slightly different definition of risk-sensitive MDP enables \emph{a stronger and more general equivalence with (reguarized) RMDP, a cleaner policy gradient theorem and better convergence property (gradient domination) as well as simpler offline RL algorithm design.}

%\yang{(proposed) The second part of this paper aims at provably efficiently solving the planning problem for a known regularized RMDP.} 
Utilizing this equivalence, we derive the policy gradient theorem for the risk-sensitive MDP problem (Theorem \ref{theorem:policy-gradient}) and prove the global convergence of the exact policy gradient method under the tabular setting with direct parameterization. Our results, to the best of our knowledge, present the first global convergence analysis with iteration complexity for a general class of risk-sensitive MDPs. Based on the policy gradient theorem, we also highlight the difficulty of gradient estimation using samples compared with the standard MDP setting.\Lina{need to revise. It reads like that suddenly we switch to risk-sensitive MDP.}

The last part of this paper is dedicated to sample-based learning for regularized RMDP. Given the challenges of sample-based gradient estimation, we consider an alternative algorithmic approach and propose a sample-based offline learning algorithm, namely the robust fitted-Z iteration (RFZI), for a specific KL-regularized RMDP problem where the regularization term is a KL-divergence term. The sample complexity for RFZI is also provided. \Lina{I forgot the details. Is the algorithm directly for risk-sensitive MDP or for regularized RMDP?} \cathy{The algorithm is directly for risk-sensitive MDP, but it might be easier to describe it as the KL-regularized RMDP?}

 Our results are verified by numerical simulations in Appendix \ref{sec:numerics}.
 




==> Sections/Intro-new.tex <==
\vspace{-10pt}
\section{Introduction}
\vspace{-5pt}
Decision-making in the face of uncertainty is a fundamental challenge across various fields such as finance \cite{follmer2016stochastic,sriboonchita2009stochastic}, engineering \citep{khan2016dynamic,shahidehpour2003market}, and robotics \citep{thrun2000probabilistic} etc. In these domains, decisions carry consequences that depend not only on expected rewards but also on the level of uncertainty or associated riskes. Addressing this challenge necessitates approaches such as robust planning, robust learning, or risk-sensitive decision-making. These approaches explicitly incorporate uncertainty and aim to find policies that perform well across a spectrum of scenarios or effectively balance the interplay between expected gains and potential risks. 


Specifically, robust Markov decision processes (RMDPs) aim to find policies that perform well under a range of possible models of the environment, rather than relying on a single assumed nominal model. This is accomplished by optimizing a worst-case objective function that considers the performance of the policy under all possible models. The RMDP framework was first introduced in \citep{iyengar2005robust,nilim2005robust}. Since then, extensive research has been conducted on RMDPs \citep{gonzalez2002minimax,xu2010distributionally,wiesemann2013robust,yu2015distributionally,mannor2016robust}, which provides
computationally efficient planning algorithms. However, these works are limited to the planning problem and do not address the challenges of reinforcement learning under model uncertainty. A few recent works have proposed robust RL algorithms with provable guarantees \citep{lim2013reinforcement,tamar2014scaling,roy2017reinforcement,badrinath2021robust,panaganti2022sample, Xu23,zhou2021finite,yang2022toward}, but most of them are either limited to
tabular and linear function approximation settings or only provide asymptotic convergence guarantees. There are also many empirical learning methods proposed to address the robust RL problem \citep{pinto2017robust,derman2018soft,mankowitz2019robust,zhang2020robust}, yet these works lack theoretical guarantees regarding algorithm convergence, sample complexity, or other performance metrics.

Risk is also an important notion that is related to robustness. The notion of coherent risk measure was first proposed and studied in financial systems \citep{artzner1999coherent,delbaen2002coherent,rockafellar2000optimization}, where the relationship to robustness is also established by characterizing risk measures as the infimum of expected shortfall over a set of probability measures (risk envelope). These works developed useful tools to evaluate the risk of uncertain outcomes. The notion of coherent risk measure is further extended to convex risk measures that can capture a broader class of risk evaluation functions \citep{follmer2002convex,ruszczynski2006optimization,follmer2002robust}. Then the conditional/dynamic risk measures are introduced to generalize the risk for a static random variable to a stochastic process with a sequence of random variables \citep{artzner2007coherent,cheridito2006dynamic,follmer2006convex,detlefsen2005conditional,riedel2004dynamic,ruszczynski2006conditional}. \citet{ruszczynski2010risk} further applies the notion of conditional coherent risk measure to MDPs and introduced the Markov risk measure. It shows that the Markov risk measure can be calculated by dynamic programming.  There is a series of follow-up works dedicated to optimizing the Markov risk measure under the RL setting \citep{ccavucs2014computational,shen2014risk,kose2021risk}, yet only asymptotic convergence results are shown. There are also works that model risks and robustness from different perspectives and settings \citep{mihatsch2002risk,fei2021risk,noorani2022risk,chow2017risk,geibel2005risk,khalil1996robust,zhang2020robust,zhang2021policy}. For instance, \citet{fei2021risk,noorani2022risk} model risk via the exponential utility, \citet{chow2017risk, geibel2005risk} consider MDP with certain performance or risk constraints, \citet{khalil1996robust, zhang2021policy} consider robustness from the robust control perspective, etc. The discussion of these settings is beyond the scope of this paper. (A more thorough summary of related literature is provided in the Appendix)

{\color{blue}
\noindent\textbf{Our Contributions:}  
In this paper, we study the iteration and sample complexity of reinforcement learning for a regularized RMDP problem, which subsumes RMDP as a special case. To gain a better understanding of the problem, we begin by introducing the risk-sensitive MDP, whose definition incorporates the concept of convex risk measures, and establishing the equivalence between these two problems (Theorem \ref{theorem:dual-representation}). We would like to emphasize that, although taken a similar recursive form, the value function for our risk-sensitive MDP is actually \emph{different} from the Markov risk measure considered in most previous literature (e.g. \citep{ruszczynski2006conditional,huang2021convergence,tamar2015policy,tamar2017sequential}, detailed elaboration in Remark \ref{rmk:difference-with-Markov-risk-measure}). This slightly different definition of risk-sensitive MDP enables \emph{a stronger and more general equivalence with (reguarized) RMDP, a cleaner policy gradient theorem and better convergence property (gradient domination) as well as simpler offline RL algorithm design.}

%\yang{(proposed) The second part of this paper aims at provably efficiently solving the planning problem for a known regularized RMDP.} 
Utilizing this equivalence, we derive the policy gradient theorem for the risk-sensitive MDP problem (Theorem \ref{theorem:policy-gradient}) and prove the global convergence of the exact policy gradient method under the tabular setting with direct parameterization. Our results, to the best of our knowledge, present the first global convergence analysis with iteration complexity for a general class of risk-sensitive MDPs. Based on the policy gradient theorem, we also highlight the difficulty of gradient estimation using samples compared with the standard MDP setting.\Lina{need to revise. It reads like that suddenly we switch to risk-sensitive MDP.}

The last part of this paper is dedicated to sample-based learning for regularized RMDP. Given the challenges of sample-based gradient estimation, we consider an alternative algorithmic approach and propose a sample-based offline learning algorithm, namely the robust fitted-Z iteration (RFZI), for a specific KL-regularized RMDP problem where the regularization term is a KL-divergence term. The sample complexity for RFZI is also provided. \Lina{I forgot the details. Is the algorithm directly for risk-sensitive MDP or for regularized RMDP?} \cathy{The algorithm is directly for risk-sensitive MDP, but it might be easier to describe it as the KL-regularized RMDP?}

 Our results are verified by numerical simulations in Appendix \ref{sec:numerics}.
 }


\subsection{\color{blue} Related Works and Comparisons}
Due to space limit, we defer a more thorough comparison of our results with previous works to the Appendix. \Lina{Is this page going to be in appendix or your even have a longer comparison in appendix?}\cathy{I plan to have a longer comparison discussing other aspects (e.g. Different objective functions, computational aspects etc.) because reviewers asked why we didn't cite those papers}
\paragraph{Relationship between risk and robustness:}  The relationship between robustness and risk for MDPs is well-studied. \cite{ruszczynski2010risk,shen2013risk, BAUERLE2022953,bauerle2022distributionally} build the equivalence between minimizing the Markov risk measure and solving a min-max Markov control problem. However, the uncertainty set (or risk envelope) for the min-max would change with the policy implemented, especially when stochastic policies are considered (see Remark \ref{rmk:difference-with-Markov-risk-measure}), which is different from the standard formulation of RMDPs, where the uncertainty sets is not related to the policy. \citep{osogami2012robustness} obtains stronger results of equivalence to RMDP yet only for certain type of risk measures such as Conditional Value at Risk (CVaR). In comparison, our proposed risk-senstive MDP can establish exact equivalence with (regularized) RMDPs for various types of coherent and convex risk measures.

There are also other works that discuss the relationship between risk and robustness under different settings or utility functions \cite{noorani2021riskrobust,noorani2022regularization,eysenbach2021maximum,derman2021twice, derman2020distributional}. In particular, \citep{derman2021twice} build the relationship of robust MDP with a certain risk-related convex programming; \citep{eysenbach2021maximum} doesn't establish exact equivalence, but rather an equivalence of a lower-bound of certain robust objective; \cite{noorani2021riskrobust,noorani2022regularization} considers exponential utility rather than Markov risk measure. 



\paragraph{Policy Gradient for Risk-Sensitive/Robust Learning:} There are many previous works focusing on applying policy gradient-based algorithm for risk-sensitive/robust learning \cite{tamar2012policy, tamar2015policy, tamar2017sequential, huang2021convergence, yu2023global, jaimungal2022robust, coache2023reinforcement, wang2022convergence,wang2022policy,kumar2023policy,li2023policy}. However, most of the works lack theoretical guarantees on the global convergence of these gradient-based algorithms \cite{tamar2012policy, tamar2015policy, tamar2017sequential,jaimungal2022robust, coache2023reinforcement}. There are some recent studies focusing on the global convergence guarantees for the policy gradient theorem. In particular, the works by \citet{huang2021convergence} and \citet{yu2023global} are most related to our work. \citet{huang2021convergence} give negative results showing that Markov risk measures are not gradient-dominant. \citet{yu2023global} prove global convergence for one specific type of risk measure - expected conditional risk measures (ECRMs). We would like to note that, enabled by the slightly different definition of risk-sensitive MDP, our policy gradient theorem takes a simpler structural form than the policy gradient considered for traditional dynamic coherent/convex risk measures \citep{tamar2012policy,coache2023reinforcement} and thus have better optimization landscape, i.e., graident domination, compared with \citep{huang2021convergence}. Given the gradient domination property, we are also able to generalize the result from \citep{yu2023global} to other type of risk measures. There are also works that considers policy gradient for RMDP with different types of uncertainty sets, for example \citet{wang2022policy} considers RMDPs with a particular R-contamination ambiguity set
\citet{kumar2023policy,li2023policy,wang2022convergence} considers policy gradient for RMDP with different uncertainty sets (e.g. s-rectangularity and non-rectangularity uncertainty set), which is out of the scope of discussion of this paper.\Lina{also the flow}

\paragraph{Offline learning for robust RL:} More and more attention are also drawn to the offline learning of robust MDP. \cite{zhou2021finite}
examined the uncertainty set defined by the KL divergence for offline data with uniformly lower bounded
data visitation distribution. \cite{shi2022distributionally} and \cite{li2022settling} provide near-optimal sample complexity bound for offline RL with weaker data coverage assumptions. However, these works focus on the limited tabular settings. \cite{ma2022distributionally} considers offline RL with linear approximation to deal with large state space, yet doesn't consider other type of possibly nonlinear approximation. Our offline algorithm is most related to the work by \citet{panaganti2022robust} where they design a fitted-Q iteration for RMDP. Our result is different from \citep{panaganti2022robust} in the following aspect: first, we consider a different uncertainty set defined via KL-divergence while they consider the uncertainty set with total variation distance; second, compare with their algorithm, which requires joint learning of two different functions, namely the robust Q function and the dual function, our algorithm is easier to implement as it only requires learning the Z function; thirdly, the assumptions in \citep{panaganti2022robust} requires not only approximate completeness for the robust Q function, but also approximate dual realizability on the dual function, whereas our assumption is weaker as it don't require the dual realizability.


\textbf{Notations.} In this paper we use $\Delta^{|\cS|}, \Delta^{|\cA|}$ to denote the probability distribution over $\cS$ and $\cA$ respectively. The notation $\Pr^{\pi,P}(s_t = s~|~s_0\sim\rho)$ is used to denote the state visitation  probability that $s_t = s$ at time step $t$ by executing policy $\pi$ for the MDP with transition model $P$. The notation $\bE_{s_t,a_t\sim \pi}$ takes the expectation over the trajectory $\{s_t,a_t\}_{t=0}^{+\infty}$ by executing policy $\pi$ with transition model $P$. We use $\<\cdot, \cdot\>$ to denote the inner product of two vectors of the same dimension.


==> Sections/Intro.tex <==
\vspace{-10pt}
\section{Introduction}
\vspace{-5pt}
Decision-making under uncertainty is a fundamental challenge in various fields such as finance \cite{follmer2016stochastic,sriboonchita2009stochastic}, engineering \citep{khan2016dynamic,shahidehpour2003market}, and robotics \citep{thrun2000probabilistic} etc. In these domains, a decision can have consequences that depend not only on its expected reward but also on the degree of model uncertainty or risks associated with them. Addressing this challenge requires approaches such as robust planning, robust learning, or risk-sensitive decision-making that explicitly account for uncertainty and aim to find policies that perform well across a range of possible models or account for the trade-off between expected reward and risk.

 %Risk-sensitive reinforcement learning, on the other hand, addresses the challenge of decision-making in situations where the consequences of a decision are not solely determined by its expected value, but also depend on the degree of risk associated with the decision. This is commonly addressed by optimizing a utility function that balances the expected value of a decision with a measure of the risk or uncertainty associated with that decision. Both robust MDPs and risk-sensitive reinforcement learning have practical applications in a wide range of fields, from finance and economics to engineering and robotics. 
%Some notable references in this area include the survey papers by Chow and Gao (2018) on robust MDPs and by Tamar et al. (2015) on risk-sensitive reinforcement learning, as well as the book by Bertsekas (2012) on dynamic programming and optimal control.


Robust Markov decision processes (RMDPs) aim to find policies that perform well under a range of possible models of the environment, rather than relying on a single assumed nominal model. This is accomplished by optimizing a worst-case objective function that considers the performance of the policy under all possible models. The RMDP framework was first introduced in \citep{iyengar2005robust,nilim2005robust}. Since then, extensive research has been conducted on RMDPs \citep{gonzalez2002minimax,xu2010distributionally,wiesemann2013robust,yu2015distributionally,mannor2016robust}, which provides
computationally efficient planning algorithms. However, these works are limited to the planning problem and do not address the challenges of reinforcement learning under model uncertainty. A few recent works have proposed robust RL algorithms with provable guarantees \citep{lim2013reinforcement,tamar2014scaling,roy2017reinforcement,badrinath2021robust,panaganti2022sample, Xu23,zhou2021finite,yang2022toward}, but most of them are either limited to
tabular and linear function approximation settings or only provide asymptotic convergence guarantees. There are also many empirical learning methods proposed to address the robust RL problem \citep{pinto2017robust,derman2018soft,mankowitz2019robust,zhang2020robust}, yet these works lack theoretical guarantees regarding algorithm convergence, sample complexity, or other performance metrics.

Risk is also an important notion that is related to robustness. The notion of coherent risk measure was first proposed and studied in financial systems \citep{artzner1999coherent,delbaen2002coherent,rockafellar2000optimization}. These works developed useful tools to evaluate the risk of uncertain outcomes. %Further, they established the relationship between risk measures and robustness via the duality theory, which suggests that every coherent risk measure has a dual representation as the supremum of certain expected value over an uncertainty set (risk envelope). 
The notion of coherent risk measure is further extended to convex risk measures that can capture a broader class of risk evaluation functions \citep{follmer2002convex,ruszczynski2006optimization,follmer2002robust}. Then the conditional/dynamic risk measures are introduced to generalize the risk for a static random variable to a stochastic process with a sequence of random variables \citep{artzner2007coherent,cheridito2006dynamic,follmer2006convex,detlefsen2005conditional,riedel2004dynamic,ruszczynski2006conditional}. \citet{ruszczynski2010risk} further applies the notion of conditional coherent risk measure to MDPs and introduced the Markov risk measure. It shows that the Markov risk measure can be calculated by dynamic programming. Further, it builds the equivalence between minimizing the Markov risk measure and solving the RMDP problem under certain assumptions. There is a series of follow-up works dedicated to optimizing the Markov risk measure under the RL setting \citep{ccavucs2014computational,shen2014risk,kose2021risk}, yet only asymptotic convergence results are shown. There are also works that model risks and robustness from different perspectives and settings \citep{mihatsch2002risk,fei2021risk,noorani2022risk,chow2017risk, geibel2005risk,khalil1996robust,zhang2020robust,zhang2021policy}. For instance, \citet{fei2021risk,noorani2022risk} model risk via the exponential utility, \citet{chow2017risk, geibel2005risk} consider MDP with certain performance or risk constraints, \citet{khalil1996robust, zhang2021policy} consider robustness from the robust control perspective, etc. The discussion of these settings is beyond the scope of this paper.

%\Lina{can you briefly mention/provide examples what are the different perspectives and settings? "For instance, they either consider **** or consider **** or ***" Your current sentence will look irresponsible to the readers }%\textcolor{blue}{TODO: other literature on risk sensitive RL}
% \citep{a2022risksensitive}: PG for risk-sensitive RL

% \citep{mihatsch2002risk,fei2021risk,noorani2022risk}: exponential criteria

% \citep{chow2017risk, geibel2005risk}: risk-constaint, control-constraint

% \citep{khalil1996robust,zhang2020robust,zhang2021policy}:lqr, robust and optimal control




%The need to put mathematical framework into the theory risk-averse preferences
%was one of motivations for the development of the general theory of risk measures.
%Starting from the seminal publication of Artzner et al. [1], the theory developed new
%tools to evaluate risk of uncertain outcomes and stochastic processes. Particularly
%relevant for us are the duality theory [1,10,15–17,34,43,45,46], and the theory of
%conditional and dynamic risk measures [2,8,11,14,18,19,28,38,48,40,45,47].

%Can follow the flow in Kishan's paper. The notion of RMDP is first proposed in .... Since then it has been intensively studied under both the planning setting and the learning setting. For the planning settings, .... Learning settings, (linear function approx or tabular)v.s. (Deep learning) , practical v.s. theoretical guarantees



%Most related literature:
%On the other hand, risk measures have been widely studied in the different settings (stochastic finance, ... cite??). cite?? established . These works focuses on the static settings. There are also a series of work that extend it to the Dynamic risk measures... 


% - A series of work about Markov risk measure: \citep{ruszczynski2010risk,kose2021risk,ccavucs2014computational}  and show that it is equivalent to robust MDP (min-max Markov control). 
\textbf{Our Contributions:}  
In this paper, we study reinforcement learning for a regularized RMDP problem, which is a generalization of the RMDP. To gain a better understanding of the problem, we begin by introducing the risk-sensitive MDP, whose definition incorporates the concept of convex risk measures, and establishing the equivalence between these two problems (Theorem \ref{theorem:dual-representation}). This result is most similar to \citep{ruszczynski2006conditional}; however, they only consider the setting with coherent risk measures, while we generalize it to convex risk measures. The equivalence offers another perspective to solve the regularized RMDP problem and provides us with more flexibility to design efficient learning algorithms for the regularized RMDP.

%\yang{(proposed) The second part of this paper aims at provably efficiently solving the planning problem for a known regularized RMDP.} 
Utilizing this equivalence, we derive the policy gradient theorem for the regularized RMDP problem (Theorem \ref{theorem:policy-gradient}) and prove the global convergence of the exact policy gradient method under the tabular setting with direct parameterization. We observe that the iteration complexity in this setting has a worse dependency on the distributional shift factor than its counterpart in the standard MDP problem, indicating that regularized RMDP optimization may be more challenging. Our results, to the best of our knowledge, present the first global convergence analysis with iteration complexity for this problem. Based on the policy gradient theorem, we also highlight the difficulty of gradient estimation using samples compared with the standard MDP setting.

The last part of this paper is dedicated to sample-based learning for regularized RMDP. Given the challenges of sample-based gradient estimation, we consider an alternative algorithmic approach and propose a sample-based offline learning algorithm, namely the robust fitted-Z iteration (RFZI), for a specific KL-regularized RMDP problem where the regularization term is a KL-divergence term. The sample complexity for RFZI is also provided.  We note that the offline learning setting for the RFZI algorithm is similar to the one considered in \cite{panaganti2022robust}, but with a different uncertainty set defined via KL-divergence. Our algorithm is easier to implement compared to \cite{panaganti2022robust} due to the equivalence between the KL-regularized RMDP and the risk-sensitve MDP with entropy risk measure.%\Lina{can we say that it is easier to implement due to the equivalence between RMDP and the risk-sensitive MDP that we establish earlier? } 
%\Lina{some discussion on the sample complexity result? compared to the literature, good or bad?}

%\Lina{a general feeling: The original contribution paragraphs, the 2nd and 3rd paragraph ignores risk-sensitive MDP totally. I added some phrases mentioning equivalence. My understanding is that both policy graident and RFZI are built for risk sensitive MDP directly. If it is the case, we can even do a better job in the 2nd and 3rd paragraph to reflect it. This also makes reviewer appreciate better of the equivalence results. }

Our results are verified by numerical simulations in Appendix \ref{sec:numerics}.


% This paper focuses on reinforcement learning with considerations of risk and robustness.
% Firstly, we present a generalization of the Markov risk measures proposed in \cite{ruszczynski2010risk} to include conditional convex risk measures in addition to the existing conditional coherent risk measures. We establish the equivalence between minimizing the generalized Markov risk measures and solving a class of regularized RMDP problems (Theorem \ref{theorem:dual-representation}). Although not a hard generalization, to our knowledge, there's no prior work that builds this equivalence. 

% Secondly, we derive the policy gradient theorem for the regularized RMDP problem (Theorem \ref{theorem:policy-gradient}) and prove the global convergence of the exact policy gradient method under the tabular setting with direct parameterization. We observe that the iteration complexity in this setting has a worse dependence on the distributional shift factor than its counterpart in the standard MDP problem, indicating that regularized RMDP optimization may be more challenging. Our results, to the best of our knowledge, present the first global convergence analysis with iteration complexity for this problem. Based on the policy gradient theorem, we also highlight the difficulty of gradient estimation using samples compared with the standard MDP setting.

% \Lina{need transition to motivate why we don't do sample based policy gradient methods} The last part of this paper is dedicated to sample-based learning for regularized RMDP. Given the challenges of sample-based gradient estimation, in this work we take a detour and seek to design the algorithm from a different perspective. We propose a sample-based offline learning algorithm, namely the robust fitted-Z iteration (RFZI), for a specific regularized RMDP problem with a KL-divergence penalty function in the regularization term. The offline learning setting for the RFZI algorithm is similar to the one considered in \cite{panaganti2022robust}, but with a different uncertainty set defined via KL-divergence. Our algorithm is easier to implement compared to \cite{panaganti2022robust} due to the special structure of the problem.

%Lastly, we developed a sample-based offline learning algorithm - robust fitted-Z iteration (RFZI) - for one specific regularized RMDP where the penalty function in the regularization term is the KL-divergence. The offline learning setting considered for the RFZI algorithm is most similar to the setting considered in \cite{panaganti2022robust}, yet they consider the RMDP setting with uncertainty set defined via total variation distance while we consider regularized RMDP with KL-divergence. Due to the special structure, our algorithm is easier to implement compared with \citep{panaganti2022robust}.% Compared with \cite{panaganti2022robust}, our algorithm is easier to implement ...

\textbf{Notations.} In this paper we use $\Delta^{|\cS|}, \Delta^{|\cA|}$ to denote the probability distribution over $\cS$ and $\cA$ respectively. The notation $\Pr^{\pi,P}(s_t = s~|~s_0\sim\rho)$ is used to denote the state visitation  probability that $s_t = s$ at time step $t$ by executing policy $\pi$ for the MDP with transition model $P$. The notation $\bE_{s_t,a_t\sim \pi}$ takes the expectation over the trajectory $\{s_t,a_t\}_{t=0}^{+\infty}$ by executing policy $\pi$ with transition model $P$. We use $\<\cdot, \cdot\>$ to denote the inner product of two vectors of the same dimension.
%\yang{We probably need a "Notations" paragraph. Symbols like $\Delta^\cS$ and $\bE_{\pi,P}$, $\Pr_{\pi,P}$ should not be defined whenever they are used.} \yang{I suggest to use notations like $\Delta^\cA$, $\bR^{\cS \times \cA}$ since we index vectors by $s$ but not by the number $i$ in $s_i$}


% \yang{I'm not sure whether this is already a convention, but the nomenclature here is actually a little confusing. MDP is the environment model we work with, while ``robust/risk-sensitive'' describes the properties of the policy/agent. The current names seem to suggest that our method only works for some specially designed envs that are designed to be robust. I would suggest ``uncertain MDP (family)'' v.s. ``robust policy optimization/robust optimal policy'' or something like that to highlight that the robustness is w.r.t. the policy.} \yang{The problem is even more obvious with risk-sensitive MDPs, since it only differs from the ``ordinary MDP'' by the objective, but objective is not part of the MDP itself.}

% \yang{If I'm to reorganize this section, I will first define MDPs and UMDPs. Then I would define the robust policy optimization problem over UMDPs, and then the regularized version for soft updates. The risk-sensitive policy optimization problem is motivated by the difficulty of implementation (?I'm not sure here) of optimization over a family of models. Then at last we provide the (restated) equivalence theorem. Also, the current organization makes our contribution unclear (it's too long for a ``problem setting'', and it's not really setting up a problem that we are going to solve). I suggest: Sec. 2 -- Prelim (MDP, UMDP, robust optim) --> regularized robust optim [new]; Sec. 3 -- prelim (risk measure, needs to be motivated) --> risk-sensitive optim [new] --> equivalence theorem [new] (emphasize that: from now on we shall focus on the risk-sensitive version that is easier to solve).}
% \Lina{For Yang's comments, I think Runyu's current flow is good. People can treat Robust MDP as a different problem as MDP. Yang's suggested flow can be taken care of in the introduction. No need to put too much words in section 2. }
